Constraining massive star activities in the final years through properties of supernovae and their progenitors

Recent observations of supernovae (SNe) just after the explosion suggest that a good fraction of SNe have the confined circumstellar material (CSM) in the vicinity, and the pre-SN enhanced mass loss may be a common property. The physical mechanism of this phenomenon is still unclarified, and the energy deposition into the envelope has been proposed as a possible cause of the confined CSM. In this work, we have calculated the response of the envelope to various types of sustained energy deposition starting from a few years before the core collapse. We have further investigated how the resulting progenitor structure would affect appearance of the ensuing supernova. While it has been suspected that a super-Eddington energy deposition may lead to a strong and/or eruptive mass loss to account for the confined CSM, we have found that a highly super-Eddington energy injection into the envelope changes the structure of the progenitor star substantially, and the properties of the resulting SNe become inconsistent with usual SNe. This argument constrains the energy budget involved in the possible stellar activity in the final years to be at most one order of magnitude higher than the Eddington luminosity. Such an energy generation however would not dynamically develop a strong wind in the time scale of a few years. We therefore propose that a secondary effect (e.g., pulsation or binary interaction) triggered by the moderate envelope inflation, which is caused by sub-Eddington energy injection, likely induces the mass loss.

==> Reply_to_report_resubmitted_to_ApJ_on_April15.tex <==
>Referee Report

>I have read the revised version of the manuscript "Constraining massive star activities in the final years through properties of supernovae and their progenitors" by Ouchi R. and Maeda K.

>It is my opinion that the modified figures and additional discussion significantly improve the clarity of the argument presented, and provide a consistent physical picture of the effects of highly super-Eddington energy deposition deep within the envelope of a red supergiant. The authors have carefully addressed all of my comments, and I believe that the paper is suitable for publication once the following minor issues are addressed.

We thank the referee for the very useful comments. We have revised the manuscript addressing all the comments.
The changes are listed below. The modified parts in the manuscript are indicated with red color.

>Section 2.1: The equation for \epsilon_inject should be labeled with an equation number.

Thank you for the comment. Following the suggestion, we have labeled the equation with an equation number.

>Table 1: I am very happy to see this table. Given that the progenitor radius used later to discuss the Popov scalings is the outermost radial coordinate of the model, it would be helpful to the reader if both the progenitor radius and the photospheric radius appear in the table.

Thank you for the suggestion. Following the suggestion, we have added the column in Table 1 for the radius of the outermost numerical cell for each model.

>Additionally, I have noticed a potential discrepancy or typographical error: The recorded photospheric radius of 3553.2 for Ldep5d39uni is much larger than both 1316.7 for the Ldep1d39uni model (with less energy deposition) and 1899.7 for the Ldep1d40uni model (with more energy deposition). The authors should check to make sure that these are the correct photospheric radii of the models. Similarly, the values for Teff, progenitor L, and Rph should be double-checked.

We have added the following sentences in the section 3.5.1:
"This can be seen by inspecting the Fig. 10 and outermost radius of the models (Rout) shown in the Table 1. Note, however, that the photospheric radius of the model Ldep1d40uni is smaller than that of Ldep5d39uni, which seems to be opposite to the intuition (see Table 1). This happens because, especially for the former model, the majority of the hydrogen envelope is recombined, and thus the photosphere recedes in radius."

During the double-checking of Teff, L, and Rph, we have realized that the luminosity in the Table1 and Fig.13 is taken at the outermost cell of the model, and not at the photosphere. We have revised the luminosity and also Teff (because Teff is calculated from L and R) to the value at the photosphere in Table1 and Fig.13. Since the change is minor, this revision does not affect our conclusion. 

Also, we found a small mistake in my code for converting the MESA progenitor model into the SNEC input style for the particular model of Ldep5d39BASE. We have rerun the calculations using the correct input model, and found that the result is almost the same as before. We have updated the Table1, Fig. 9, and Fig.14 using the correct result for Ldep5d39BASE, although the change is hardly discernable.

Apart from the two caveats described above, we have confirmed that the Rph in Table 1 are the correct values.

>Table 1f: Typographical error "...where the specific total energy is negative" should be "... where the specific total energy is positive" if this describes mass that is unbound.

Thank you for pointing out this. We have corrected the word "negative" to "positive".

>It could also be clarified when discussing this in the text what region of the star this mass is contained in. Is this outside the photosphere, or is this in the inner region where energy is being deposited, which may be surrounded on either end by bound material?

We have added the following sentences in the section 3.1:
"Also, the inner radius of the unbound region is well within the photosphere for all the models that have unbound mass. For the model of Ldep5d39uni, for example, the inner radius of the unbound region is 171.9Rsun, which is much smaller than the photospheric radius. Thus, the photosphere resides in the unbound region."

>Section 3.3: Regarding the added text: "This is because the shock velocity is decelerated when the shock hits the high density shell..." While this does occur, I do not believe it is a complete explanation for the lowered velocity, and would be careful not to lend too much physical significance to the density inversion outside the photosphere. It is likely that this lower velocity can also be explained by shock deceleration as it travels into a radially extended envelope, following Matzner & McKee (1999 - doi:10.1086/306571). Shock velocity scales inversely with radius and more weakly with density (Equation 19, vshock \propto (rho r^3)^-0.19, also Equation 32 in the fourth MESA instrument paper, Paxton et al 2018). Because of this, I believe the photospheric velocity at early times, which describes material near the outermost ejecta because the photospheric temperature remains above the H recombination temperature, is lower at least in part because the shock has travelled farther radially outward and is therefore weaker. I do not believe that all of this detail must be stated; adding a brief sentence along the lines of "Additionally, the shock has travelled farther radially outward, which also leads to lower velocity in the outermost ejecta (Matzner & McKee 1999)." would suffice. 

Thank you for the constructive comments. Following the suggestion, we added the following sentence:
"Additionally, the shock has travelled farther radially outward, which also leads to lower velocity in the outermost ejecta (Matzner & McKee 1999)."

>Section 4.1 : It would be helpful if the Popov scalings were typeset as equations and labeled with equation numbers.

Thank you for the suggestion. Following the suggestion, we have typeset the scalings with equation numbers.

>Section 4.2: Regarding the text "CSM within a few years with the mass flux of Mdot...": I find the term "mass flux" confusing when in this specific context (but helpful throughout the rest of the text), given that the literature generally discusses mass loss, even though the two are taken to mean roughly the same thing in this work. A way around this here would be to say "CSM within a few years with the mass flux out of the star of Mdot =...", or even simply "CSM within a few years with Mdot =...".

Thank you for the suggestion. Following the suggestion, we have rewritten the sentence as "CSM within a few years with Mdot =...".

>Section 4.4: It is unclear to me what is meant by "feedback" in "Also the feedback from the change in the density structure may not be negligible". This could be clarified.

Thank you for the suggestion. Following the suggestion, we have rewritten the sentence as:
"Also, the change of the density structure by the energy deposition might suppress the fraction of the wave power that can tunnel to the envelope (Quatart & Shiode 2012)"

>Abstract and conclusions: "This argument constrains the energy budget involved in the possible stellar activity in the final years to be at most comparable to or less than the Eddington luminosity" no longer appears to be accurate if taken at face value, as an injection of 1e39 erg/s, which is certainly greater than the (revised) Eddington luminosity of ~10^38 ergs/s, does not lead to dramatic differences in the supernova observables. However, "comparable to" could leave room for interpretation. Therefore I leave it up to the authors to what extent they would like to qualify this claim.

Thank you for the comment. We have rewritten the sentences in the abstract and conclusion as follows:
- Abstract:
"This argument constrains the energy budget involved in the possible stellar activity in the final years to be at most one order of magnitude higher than the Eddington luminosity."

- Conclusion:
"We have also found that if highly super-Eddington energy deposition takes place, which exceeds the Edding- ton luminosity by more than an order of magnitude,..."
"On the contrary, if the energy injection rate is moderate and does not exceed the Eddington luminosity by more than one order of magnitude, the envelope expands..."

